Submodular Maximization over Sliding Windows

In this paper we study the extraction of representative elements in the data stream model in the form of submodular maximization. Different from the previous work on streaming submodular maximization, we are interested only in the recent data, and study the maximization problem over sliding windows. We provide a general reduction from the sliding window model to the standard streaming model, and thus our approach works for general constraints as long as there is a corresponding streaming algorithm in the standard streaming model. As a consequence, we obtain the first algorithms in the sliding window model for maximizing a monotone/non-monotone submodular function under cardinality and matroid constraints. We also propose several heuristics and show their efficiency in real-world datasets.

==> conclude.tex <==
\section{conclusion}

==> swdp.tex <==
\subsection{The DP-based Greedy Algorithm}
\label{sec:greedy}

In this section we prove the following theorem for maximizing \emph{monotone} submodular function subject to cardinality constraint $k$.
\begin{theorem}
\label{thm:greedy}

There is an algorithm for cardinality constrained monotone submodular maximization over sliding windows that achieves a $(1/2-\eps)$-approximation using $O(k^2/\eps \cdot \log M)$ words of space and $O(k/\eps \cdot \log M)$ update time (in terms of number of function calls) per item.
\end{theorem}


\begin{algorithm2e}[t]
\DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
\KwIn{$k$ the cardinality constraint; $W$: the size of the window; $T$ the threshold. }
%\KwOut{}
%\tcc{}


\ForEach{$j = 0, 1, \ldots, k$}{
  $(\ell_j, S_j) \gets (-1, \emptyset)$
}

\ForEach{new incoming element $e_i$}{
  set $(\ell_0, S_0) \gets (i, \emptyset)$\;
  \ForEach{$j = 0, 1, \ldots, k$}{
    \If{$\ell_j \le i - W$}{
      set $\ell_j \gets -1$
    }
  }
  \ForEach{$j = 0, 1, \ldots, k$ s.t. $\ell_j \neq -1$}{ \label{line:loop}
    \If{$f(e_i | S_j) \ge T$ and $\ell_j > \ell_{j+1}$}{ \label{line:conditions}
      set $\ell_{j+1} \gets \ell_j$, and $S_{j+1} \gets S_j \cup \{e_i\}$
    }
  }
}

\Return{(at query) $S_{j_{\max}}$ where $j_{\max} = \max\{j ~|~ 0 \leq j \leq k, j \neq -1\}$}
\caption{\thresh($k, W, T$)}
\label{alg:greedy-thresh}
\end{algorithm2e}


\begin{algorithm2e}[t]
\DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
\KwIn{$k$ the cardinality constraint;  $W$: the size of the window; $M$: an upper bound of $f(\OPT)$ over sliding windows.}
%\KwOut{}
%\tcc{}
$L \gets 1 + \log_{1+\eps}M$\;

\ForEach{$T = \frac{(1 + \eps)^0}{2k}, \frac{(1 + \eps)^1}{2k},  \ldots, \frac{(1 + \eps)^L}{2k}$}{
  create an instance of \thresh$(k, W, T)$ 
}
run all created instances in parallel\;
\Return{(at query) the best solution among those returned by all instances}
\caption{\swdp$(k, W, M)$}
\label{alg:greedy}
\end{algorithm2e}


The pseudocode of the algorithm is described in Algorithm~\ref{alg:greedy-thresh} and Algorithm~\ref{alg:greedy}. We run instances of \thresh\ for different thresholds. For a fixed threshold $T$, we maintain $\ell_j$ and $S_j$ for each $0 \leq j \leq k$, where $\ell_j$ is the last starting time step such that we still manage to get $j$ elements (denoted by $S_j$) passing $T$. Upon receiving a new element $e_i$, we set $(\ell_0, S_0) \gets (i, \emptyset)$ and drop all the expired $\ell_j$'s by marking their values to be $-1$. Finally for all the active $\ell_j$'s, we use the conditions in Line \ref{line:conditions} of Algorithm \ref{alg:greedy-thresh} to decide if the value of $(\ell_j, S_j)$ needs to be updated.

We create $L = O(\eps^{-1}\log M)$ instances of \thresh, and each instance tracks $\ell_j$ and $S_j$ for all $0 \leq j \leq k$. Together with the fact that each $S_j$ uses $O(k)$ words, the space usage is bounded by $O(\eps^{-1}k^2\log M)$. The update time is straightforward once we note that in each instance of \thresh, $j$ loops from $0$ to $k$ for every item in Line \ref{line:loop} of Algorithm \ref{alg:greedy-thresh}. 


We next prove the correctness of our algorithm. Consider the choice of $T$ satisfying
\begin{equation}
  \label{eq:T-ineq}
  f(\OPT)/(2k) \le T \le (1+\eps) f(\OPT) / (2k).
\end{equation}
Let $j_{\max} = \max\{j ~|~ 0 \leq j \leq k, \ell_{j} \neq -1\}$.  If $j_{\max} = k$, then we must have $f(S_{j_{\max}}) \ge T \cdot k \ge f(\OPT)/2$.  We now consider the case when $j_{\max} < k$.   It is easy to see that for all $e \in \OPT \setminus S_{j_{\max}}$, when they are considered to be added to a predecessor $S_{j_e}$ of $S_{j_{\max}}$ (thus $S_{j_e} \subseteq S_{j_{\max}}$), they are rejected.  Note that they cannot be rejected by the check $\ell_{j_e} > \ell_{j_e+1}$, since otherwise by the definition $\ell_{j_e}$ can never be part of the best solution. We thus must have $f(e|S_{j_e}) < T$. By submodularity, we have
\begin{eqnarray}
f((\OPT\setminus S_{j_{\max}}) \cup S_{j_{\max}}) - f(S_{j_{\max}}) &\le& \sum_{e \in \OPT\setminus S_{j_{\max}}} f(e | S_{j_{\max}}) \nonumber \\
&\le& \sum_{e \in \OPT\setminus S_{j_{\max}}} f(e | S_{j_e}) \leq  kT \nonumber \\
&\le& (1+\eps)f(\OPT)/2. \label{eq:a-1}
\end{eqnarray}
On the other hand, 
\begin{equation}
\label{eq:a-2}
f((\OPT\setminus S_{j_{\max}})\cup S_{j_{\max}}) = f(\OPT \cup S_{j_{\max}}) \ge f(\OPT).
\end{equation}
By (\ref{eq:a-1}) and (\ref{eq:a-2}) we have $f(S_{j_{\max}}) \ge (1-\eps)f(\OPT)/2$.  

Therefore, for any sliding window query, the solution returned by \swrd\ is no worse than $(1-\eps)f(\OPT)/2$. This is because we always have an instance of \thresh\ that uses a thresh $T$ satisfying (\ref{eq:T-ineq}).

